Class-Aware Fully-Convolutional Gaussian and Poisson Denoising

We propose a fully-convolutional neural-network architecture for image denoising which is simple yet powerful. Its structure allows to exploit the gradual nature of the denoising process, in which shallow layers handle local noise statistics, while deeper layers recover edges and enhance textures. Our method advances the state-of-the-art when trained for different noise levels and distributions (both Gaussian and Poisson). In addition, we show that making the denoiser class-aware by exploiting semantic class information boosts performance, enhances textures and reduces artifacts.

==> experiments_agnostic_old.tex <==
In all experiments in this section a separate network was trained for each noise type and level using $8K$ images from the PASCAL VOC \cite{everingham2010pascal} according to the methodology explained in Section \ref{sec_method_agnostic}. Performance was evaluated on the following test sets: (i) images from PASCAL VOC \cite{pascal-voc-2010}; and (ii) the commonly used $68$ test images chosen by \cite{roth2009fields} from the Berkeley segmentation dataset \cite{MartinFTM01}. (iii) In the case of Poisson noise we additionally evaluated performance on a commonly used test set of $10$ images. 

While applying Gaussian noise with a sigma ranging from $10$ up to $75$ our network was compared to (a) BM3D ;(b) multilayer perceptrons (MLP) using sigma specific, pre-trained models trained on ImageNet and made available online; and (c) TNRD using sigma specific, pre-trained models published by the authors;

In the Poisson case, for peak value ranging from $1$ up to $30$ we compared our method to (a) I+VST+BM3D; \tal{add the rest of the methods}. Whenever code for other techniques was not publicly available, we evaluated our method on the same test set and compared with their reported scores.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{PASCAL VOC}
\label{sec_agnostic_pascal}
In this experiment we tested the denoising algorithms on $1K$ test images from \cite{pascal-voc-2010}.

Table \ref{tab_pascal_gaussian} summarizes performance in terms of average PSNR for white Gaussian noise and Table \ref{tab_pascal_poisson} does so for the Poisson noise.

\begin{table}[h!]
\centering
\small
\begin{tabular}{ l@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c  }
    \hline\hline
    $\sigma$					& $10$ & $15$ & $25$ & $35$ & $50$ & $65$ & $75$ \\ \hline
    BM3D						& $34.26$ & $32.10$ & $29.62$ & $28.14$ & $26.61$ & $25.64$ & $25.12$ \\  
    MLP \cite{burger2012image} 	& $34.29$ & $-$ & $29.95$ & $28.49$ & $26.98$ & $26.07$ & $25.54$ \\  
    TNRD \cite{Chen16Trainable}	& $-$ & $32.35$ & $29.90$ & $-$ & $26.91$ & $-$ & $-$ \\  
    DenoiseNet 					& $\textbf{34.87}$ & $\textbf{32.79}$ & $\textbf{30.33}$ & $\textbf{28.88}$ & $\textbf{27.32}$ & $\textbf{26.30}$ & $\textbf{25.75}$	\\ \hline \hline
  \end{tabular}  
  \vspace{2mm}
\caption{\small \textbf{PASCAL VOC - Gaussian noise} Average PSNR values on a $1000$ image test set.}
\label{tab_pascal_gaussian}	
\end{table}

\begin{table}[h]
\centering
  \begin{tabular}{ l@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c  }
    \hline \hline
    	Peak 		& $1$ 	& $2$ 	& $4$ 	& $8$ 	& $30$ \\ \hline
		I+VST+BM3D  & $22.71$ & $23.70$ 	& $24.78$ 	& $26.08$ 	& $28.85$ \\
    	DenoiseNet    & $\textbf{22.87}$ & $\textbf{24.09}$ 	& $\textbf{25.36}$ 	& $\textbf{26.70}$ 	& $\textbf{29.56}$ \\
     \hline\hline
  \end{tabular}  
  \vspace{2mm}
\caption{\small \textbf{PASCAL VOC - Poisson noise} Average PSNR values for different peak values on $1000$ test images and $15$ noise realizations per image.} 
\label{tab_pascal_poisson}	
\end{table}

Figure \ref{pascal_s_curve_g} examines the statistical significance of the improvement our method achieves for Gaussian noise with $\sigma=25$. It compares the gain in performance with respect to BM3D achieved by our method, MLP and TNRD. The plot visualizes the large and consistent improvement in PSNR achieved by our method and that it outperforms all others on $92.4\%$ of the images, whereas MLP, BM3D, and TNRD win on $6.6\%, 1\%$ and $0\%$ respectively. For the Poisson noise we compare in Figure \ref{} the gain in performance with respect to I+VST+BM3D. In this case the comparison is done for multiple peak values. In both figures image indices are sorted in ascending order of performance gain. A small zero-crossing value affirms our method outperforms others on the large majority of the images in the dataset. The plots visualizes the significant and consistent improvement in PSNR achieved by our method in both presented scenarios.

\begin{figure}[tbh] 
\includegraphics[width=0.48\textwidth]{pascal_s_curve_gaussian.eps}
\caption{\small\textbf{Gaussian noise performance profile relative to BM3D.}  Image indices are sorted in ascending order of performance gain relative to BM3D. The improvement of our method is demonstrated by (i) decrease of the zero-crossing point, and (ii) consistently higher values of gain. The comparison was made on images from PASCAL VOC for $\sigma=25$.}
\label{pascal_s_curve_g}
\end{figure} 

\begin{figure}[t] 
\includegraphics[width=0.48\textwidth]{pascal_s_curve_poisson.eps}
\caption{\textbf{Poisson noise performance profile relative to I+VST+BM3D \cite{Azzari16Variance}.}  Image indices are sorted in ascending order of performance gain relative to I+VST+BM3D. The improvement of our method is demonstrated by (i) small zero-crossing point, and (ii) consistently higher PSNR values. The distribution reveals the statistical significance of the reported improvement. The comparison was made on images from PASCAL VOC and $15$ noise realizations per image.} 
\label{pascal_s_curve}
\end{figure} 


\tal{add some images for example if space permits}
%Denoising of several images from the test-set are visualized in Figure \ref{fig_large_pascal}. We encourage the reader to zoom-in to appreciate the significant improvement our method achieves, resulting in much more aesthetically pleasing images.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Berkeley segmentation dataset}
\label{sec_agnostic_berkeley}
In this experiment we tested the performance of our method, trained on PASCAL VOC, on the widely used test-set of $68$ images selected by \cite{roth2009fields} from Berkeley segmentation dataset \cite{MartinFTM01}. Even though these test images belong to a different dataset, Table \ref{tab_bsds_nonquantized_results} shows that our method outperforms previous methods for all $\sigma$ values.
%
\begin{table}[h!]
\centering
\small
\begin{tabular}{ l@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c@{\hskip 0.01\textwidth}c  }
    \hline\hline
    $\sigma$					& $10$ & $15$ & $25$ & $35$ & $50$ & $65$ & $75$ \\ \hline
    BM3D						& $33.31$ & $31.10$ & $28.57$ & $27.08$ & $25.62$ & $24.68$ & $24.20$ \\  
    MLP \cite{burger2012image} 	& $33.50$ & $-$ & $28.97$ & $27.48$ & $26.02$ & $25.10$ & $24.58$ \\  
    TNRD \cite{Chen16Trainable}	& $-$ & $31.41$ & $28.91$ & $-$ & $25.95$ & $-$ & $-$ \\  
    DenoiseNet 					& $\textbf{33.58}$ & $\textbf{31.44}$ & $\textbf{29.04}$ & $\textbf{27.56}$ & $\textbf{26.06}$ & $\textbf{25.12}$ & $\textbf{24.61}$	\\ \hline \hline
  \end{tabular}   
  \vspace{2mm}
\caption{\small \textbf{Performance on images from Berkeley segmentation dataset.} Average PSNR values on a test set of $68$ images selected by \cite{roth2009fields}. Our method outperforms all others for all noise levels.
\vspace{-4mm}}
\label{tab_bsds_nonquantized_results}	
\end{table}


==> video_25_figure.tex <==

\begin{figure*}[bt]
	\centering	
    \small    
    \begin{tabular}{m{0.15\textwidth}@{\hskip 0.005\textwidth}K{0.27\textwidth}@{\hskip 0.005\textwidth}K{0.27\textwidth}@{\hskip 0.005\textwidth}K{0.27\textwidth}}
    	& $t=t_0-1$ & $t=t_0$ & $t=t_0+1$ \\

		Ground truth &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_769_gt.jpg} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_770_gt.jpg} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_771_gt.jpg} \\

        I+VST+BM3D &
        &
        &
        \\
        
        vBM4D &
        &
        &
        \\

        Ours $T=1$ &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_769_seq_1.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_770_seq_1.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_771_seq_1.png} \\
        
        Ours $T=5$ &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_769_seq_5.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_770_seq_5.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_771_seq_5.png} \\

        Ours $T=11$ &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_769_seq_11.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_770_seq_11.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_25_771_seq_11.png} \\
	\end{tabular}   \\
	\caption{\small\textbf{Video denoising examples for peak value 30.} Presented are three consecutive images from video $\#1$ at times $t_0, t_0-1$, and $t_0+1$. The top row presents the ground truth images, each of the following rows present the output of a different denoising method. All image intensities have been linearly stretched to enable better viewing.}
    \label{fig_denoise_vid_1}
\end{figure*}

==> video_5_figure.tex <==

\begin{figure*}[bt]
	\centering	
    \small    
    \begin{tabular}{m{0.15\textwidth}@{\hskip 0.005\textwidth}K{0.27\textwidth}@{\hskip 0.005\textwidth}K{0.27\textwidth}@{\hskip 0.005\textwidth}K{0.27\textwidth}}
    	& $t=t_0-1$ & $t=t_0$ & $t=t_0+1$ \\

		Ground truth &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_434_gt.jpg} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_435_gt.jpg} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_436_gt.jpg} \\

        I+VST+BM3D &&&\\
        
        vBM4D &&& \\

        Ours $T=1$ &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_434_seq_1.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_435_seq_1.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_436_seq_1.png} \\
        
        Ours $T=5$ &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_434_seq_5.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_435_seq_5.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_436_seq_5.png} \\

        Ours $T=11$ &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_434_seq_11.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_435_seq_11.png} &
        \includegraphics[width = 0.27\textwidth]{./figures/vid_5_436_seq_11.png} \\
	\end{tabular}   \\
	\caption{\small\textbf{Video denoising examples for peak value 30.} Presented are three consecutive images from video $\#1$ at times $t_0, t_0-1$, and $t_0+1$. The top row presents the ground truth images, each of the following rows present the output of a different denoising method. All image intensities have been linearly stretched to enable better viewing.}
    \label{fig_denoise_vid_1}
\end{figure*}
